SNARKs to the rescue: proof-of-contact in zero knowledge

This paper describes techniques to help with COVID-19 automated contact tracing, and with the restoration efforts. We describe a decentralized protocol for ``proof-of-contact'' in zero knowledge where a person can publish a short cryptographic proof attesting to the fact that they have been infected and that they have come in contact with a set of people without revealing any information about any of the people involved. More importantly, we describe how to compose these proofs to support broader functionality such as proofs of $n$th-order exposure which can further speed up automated contact tracing. The cryptographic proofs are publicly verifiable, and places the burden on the person proving contact and not on third parties or healthcare providers rendering the system more decentralized, and accordingly more scalable.

==> immunity.tex <==
\section{Proofs of Health / Immunity}
The same technique may be used by Alice to prove she is healthy i.e., she received a negative test from her healthcare provider within the past day or week. The same is true for proving immunity with the antibodies test that is gaining traction as communities look towards restoration. For example, a proof-of-health would consist of a zkSNARK attesting that:
\begin{itemize}
    \item  $h_s=H(S, \mathsf{COVID.negative}, t')$
    \item $t - t' \leq 1$ day 
\end{itemize}

Here the value $t$ is a public value such as the current day, whereas the value $t'$ is private and represents the date of the negative test result. The user then provides the tuple $(\pi, h_s, s, t)$ to the verifier.

We note that in general, this protocol might is not a sufficient for implementation of "immunity passports." The non-interactive proofs are susceptible to replay attacks e.g., Alice could provide a proof to Bob, who later provides the same proof to Charlie. Since the zkSNARKs are anonymous proofs, there is no verification of identity. In this sense, we believe an interactive protocol is better suited. 

\subsection{Ethics of "Immunity Passports"}
